Mass Production of 2023 KMTNet Microlensing Planets I: Low Mass Ratio

We initiate the systematic search for planets in the 2023 data of the Korea Microlensing Telescope Network (KMTNet), focusing on those planets found by the KMTNet AnomalyFinder with low preliminary estimates of the mass-ratio, $q<2\times 10^{-4}$. The 2023 season is the first for which the photometry of all events was re-reduced prior to the AnomalyFinder search, potentially increasing its sensitivity to planets. We find three strong low-$q$ planet candidates, KMT-2023-BLG-0164 ($q\sim 1.3\times 10^{-4}$), KMT-2023-BLG-1286 ($q\sim 1.9\times 10^{-4}$), and KMT-2023-BLG-1746 ($q\sim 8\times 10^{-5}$). KMT-2023-BLG-0164 is notable in that the source is projected on a very bright ($I=16.0$) foreground star, which is either the planet's host or (more likely) a companion to the host. We obtain a spectrum, finding that its mass and distance are $M\sim 1.0\,M_\odot$ and $D\sim 1.5$ kpc, the latter being the distance of the lens ($D_L$) regardless of whether the spectroscopic target is the host or its companion. We also analyze two other candidates, KMT-2023-BLG-0614 and KMT-2023-BLG-1593, which are unlikely to enter the statistical sample due to their ambiguous interpretations as possible non-planetary events.

==> tabnames.tex <==
 \begin{deluxetable}{lrrrrrr}
 \tablecolumns{7} \tablewidth{0pc}
 \tablecaption{\textsc{Event Names, Cadences, Alerts, and Locations}}
 \tablehead{\colhead{Name} & 
\colhead{$\Gamma\,({\rm hr}^{-1})$} &
\colhead{Alert Date} &
\colhead{RA$_{\rm J2000}$} &
\colhead{Dec$_{\rm J2000}$} &
\colhead{$l$} &
\colhead{$b$} }
%\hline
 \startdata
KMT-2023-BLG-0164 & 2.4 & 27 Mar 2023 & 17:59:11.98 & $-$31:46:14.41 & $-0.95$ & $-3.96$\\ % 14.50
OGLE-2023-BLG-0116 & 0.1\\
MOA-2023-BLG-107 & 1.2\\
\hline
KMT-2023-BLG-1286 & 4.0 & 19 Jun 2023 & 18:05:28.46 & $-$27:52:11.32 & $+3.12$ & $-3.23$\\ %14.35
OGLE-2023-BLG-0803 & 1.0\\
\hline
KMT-2023-BLG-1746 & 0.4 & 19 Jul 2023 & 17:48:38.60 & $-$35:17:53.09 & $-5.11$ & $-3.84$\\ % 14.62
\hline
KMT-2023-BLG-0614 & 2.0 & 28 Apr 2023 & 17:57:19.04 & $-$27:55:27.19 & $+2.19$ & $-1.69$\\ % 14.37
\hline
KMT-2023-BLG-1593 & 4.0 & 10 Jul 2023 & 17:54:34.33 & $-$28:24:47.12 & $+1.46$ & $-1.42$\\ % 14.38
\hline
 \enddata
 \tablecomments{The coordinates given here are for the nearest catalog 
   stars (i.e., baseline objects).
   %In Section~\ref{sec:cmd} we discuss the offsets from these locations of the actual events.
}
 \label{tab:names}
 \end{deluxetable}


